Hyper-differential sensitivity analysis in the context of Bayesian inference applied to ice-sheet problems

Inverse problems constrained by partial differential equations (PDEs) play a critical role in model development and calibration. In many applications, there are multiple uncertain parameters in a model which must be estimated. Although the Bayesian formulation is attractive for such problems, computational cost and high dimensionality frequently prohibit a thorough exploration of the parametric uncertainty. A common approach is to reduce the dimension by fixing some parameters (which we will call auxiliary parameters) to a best estimate and use techniques from PDE-constrained optimization to approximate properties of the Bayesian posterior distribution. For instance, the maximum a posteriori probability (MAP) and the Laplace approximation of the posterior covariance can be computed. In this article, we propose using hyper-differential sensitivity analysis (HDSA) to assess the sensitivity of the MAP point to changes in the auxiliary parameters. We establish an interpretation of HDSA as correlations in the posterior distribution. Our proposed framework is demonstrated on the inversion of bedrock topography for the Greenland ice sheet with uncertainties arising from the basal friction coefficient and climate forcing (ice accumulation rate)

==> main_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
%\usepackage{algorithm2e}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps
\fi
%\usepackage{amsmath,amssymb, amsfonts}
%\usepackage{algorithm}
\usepackage{float}
%\usepackage{subcaption}
% \usepackage{relsize}
\usepackage{graphicx}
\usepackage{booktabs} 
%\usepackage[table]{xcolor}
\usepackage{bm}
\usepackage{setspace}
%\usepackage{amsthm}
\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{algorithm}
\usepackage[mathscr]{euscript}
%\usepackage{algpseudocode}
\usepackage{cite}
\usepackage{comment}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newtheorem{assumption}{Assumption}

\newsiamthm{prop}{Proposition}
\newsiamthm{example}{Example}
\DeclareMathOperator*{\argmax}{arg\,max}
\renewcommand{\vec}[1] {\ensuremath{\boldsymbol{#1}}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

\newcommand{\joeynote}[1]{{\color{red}Joey : {#1}}}
\newcommand{\bartnote}[1]{{\color{blue}Bart : {#1}}}

% Sets running headers as well as PDF title and authors
%\headers{HDSA for model discrepancy}{J. Hart and B. van Bloemen Waanders}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{Hyper-differential sensitivity analysis with respect to model discrepancy: Calibration and Optimal Solution Updating \thanks{Submitted to the editors DATE.}}

% Authors: full names plus addresses.
%\author{Joseph Hart\thanks{Scientific Machine Learning, Sandia National Laboratories, P.O. Box 5800, Albuquerque, NM 87123-1320
%  (\email{joshart@sandia.gov}).}
%\and Bart van Bloemen Waanders \thanks{Scientific Machine Learning, Sandia National Laboratories, P.O. Box 5800, Albuquerque, NM 87123-1320
%  (\email{bartv@sandia.gov}).} }

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\def\R{{\mathbb R}}
\def\U{{\mathcal U}}
\def\Z{{\mathcal Z}}
\def\t{{\vec{\theta}}}
\def\u{{\vec{u}}}
\def\c{{\vec{c}}}
\def\z{{\vec{z}}}
\def\zbar{{\overline{\z}}}
\def\x{{\vec{x}}}
\def\e{{\vec{e}}}
\def\v{{\vec{v}}}
\def\w{{\vec{w}}}
\def\y{{\vec{y}}}
\def\s{{\vec{s}}}
\def\a{{\vec{a}}}
\def\b{{\vec{b}}}
\def\J{{\vec{J}}}
\def\c{{\vec{c}}}
\def\d{{\vec{\delta}}}
\def\A{{\vec{A}}}
\def\B{{\vec{B}}}
\def\E{{\vec{E}}}
\def\M{{\vec{M}}}
\def\K{{\vec{K}}}
\def\G{{\vec{G}}}
\def\S{{\vec{S}}}
\def\N{{\vec{N}}}
\def\L{{\vec{L}}}
\def\C{{\vec{C}}}
\def\D{{\vec{D}}}
\def\H{{\vec{H}}}
\def\P{{\vec{P}}}
\def\Q{{\vec{Q}}}
\def\X{{\vec{X}}}
\def\V{{\vec{V}}}
\def\q{{\vec{q}}}
\def\I{{\vec{I}}}
\def\g{{\vec{g}}}
\def\W{{\vec{W}}}
\def\T{{\vec{T}}}
\def\Y{{\vec{Y}}}
\def\F{{\vec{F}}}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\def\b{{\vec b}}
\def\z{{\vec z}}
\def\t{{\vec \theta}}
\def\r{{\mathbb R}}
\def\d{{\vec d}}
\def\e{{\vec e}}
\def\f{{\vec f}}
\def\g{{\vec g}}
\def\F{{\vec F}}
\def\noise{{\vec \eta}}
\def\y{{\vec y}}
\def\w{{\vec w}}
\def\u{{\vec u}}
\def\v{{\vec v}}
\def\s{{\vec s}}
\def\m{{\vec m}}
\def\ltwo{{L^2(\Omega)}}
\def\gaussian{{\mathcal N}}
\def\zero{{\vec 0}}
\def\mgamma{{\vec \Gamma}}
\def\likelihood{{\pi_\text{like}}}
\def\x{{\vec x}}

\def\rq{\mathbb{R}^q}
\def\real{\mathbb{R}}
\def\rd{\mathbb{R}^d}
\def\vnoise{{\vec \eta}}
\def\forcing{h_{\text{flux}}}

\def\Aop{\boldsymbol{\mathcal{A}}}
\def\Bop{\boldsymbol{\mathcal{B}}}
\def\Cop{\boldsymbol{\mathcal{C}}}
\def\Gop{\boldsymbol{\mathcal{G}}}
\def\Hop{\boldsymbol{\mathcal{H}}}
\def\Pop{\boldsymbol{\mathcal{P}}}
\def\Vop{\boldsymbol{\mathcal{V}}}

\def\mass{{\vec M}}
\def\stiff{{\vec K}}
\def\ma{{\vec A}}
\def\mb{{\vec B}}
\def\mc{{\vec C}}
\def\ml{{\vec L}}
\def\mh{{\vec H}}
\def\mi{{\vec I}}
\def\my{{\vec Y}}
\def\mx{{\vec X}}
\def\ms{{\vec S}}
\def\md{{\vec D}}
\def\mt{{\vec T}}
\def\mj{{\vec J}}
\def\mv{{\vec V}}
\def\mlambda{{\vec \Lambda}}
\def\momega{{\vec \Omega}}
\def\mq{{\vec Q}}
\def\pN{\mathcal{N}}

\newcommand{\nbbd}[1]{\mathcal{N}(#1)}
%\newcommand{\V}[1]{\boldsymbol{#1}}
%\newcommand{\M}[1]{\boldsymbol{#1}}
\newcommand{\Mc}[1]{\boldsymbol{\mathcal{#1}}}
\newcommand{\thetabar}{\overline{\vec{\theta}}}
\newcommand{\bmat}[1]{\begin{bmatrix}#1 \end{bmatrix}}

\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

